An Information-Theoretic Perspective on Variance-Invariance-Covariance Regularization

Variance-Invariance-Covariance Regularization (VICReg) is a self-supervised learning (SSL) method that has shown promising results on a variety of tasks. However, the fundamental mechanisms underlying VICReg remain unexplored. In this paper, we present an information-theoretic perspective on the VICReg objective. We begin by deriving information-theoretic quantities for deterministic networks as an alternative to unrealistic stochastic network assumptions. We then relate the optimization of the VICReg objective to mutual information optimization, highlighting underlying assumptions and facilitating a constructive comparison with other SSL algorithms and derive a generalization bound for VICReg, revealing its inherent advantages for downstream tasks. Building on these results, we introduce a family of SSL methods derived from information-theoretic principles that outperform existing SSL techniques.

==> 5_acknowledgements.tex <==
\section*{Acknowledgments}

Tim G. J. Rudner is funded by a Qualcomm Innovation Fellowship.

==> include/custom.tex <==
%%%%%%% USEPACKAGES

\usepackage[utf8]{inputenc}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{booktabs} % for professional tables
\usepackage{titletoc}
\usepackage{hyperref}

\usepackage{amsmath}
% \usepackage{amsthm}
\usepackage{amssymb}
\usepackage{bbm} 
\usepackage{bm}
\usepackage{verbatim}
\usepackage{float}
\usepackage{color,soul}
\usepackage{enumitem}
\usepackage{mathtools}
\usepackage{hhline}
\usepackage[title]{appendix}
% \usepackage{natbib}
\usepackage[nameinlink]{cleveref} % MUST be added last to work properly
%\usepackage{cite}
%\usepackage{autonum}
%\usepackage[super,negative]{nth}
% \usepackage[font=small,labelfont=bf,
%    justification=justified,
%    format=plain]{caption}
% \usepackage{subcaption}
% \usepackage{tabularx}
\usepackage{tikz}
\usepackage{wrapfig,booktabs}
\usepackage{xspace}
\usepackage{cancel}
\usepackage{sidecap}
% \usepackage{authblk}

\graphicspath{ {../figures/} }

%%%%%%% LAYOUT

% \newenvironment{keywords}
% {\bgroup\leftskip 20pt\rightskip 20pt \small\noindent{\bf Keywords:} }%
% {\par\egroup\vskip 0.25ex}



%%%%%%% CUSTOM FUNCTIONS

\def\UrlBreaks{\do\/\do-}  % breaks URLs at hyphens
% \usepackage[hyphenbreaks]{breakurl}
% \hypersetup{breaklinks=true}
% \urlstyle{same}

% For operators/commands with two arguments
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}


%%%%%%% COMMENTS
\newcommand{\cmt}[1]{{\footnotesize\textcolor{red}{#1}}}
\newcommand{\note}[1]{\cmt{Note: #1}}
\newcommand{\question}[1]{\cmt{\textbf{Question}: #1}}
% \newcommand{\todo}[1]{\cmt{TO-DO: #1}}


%%%%%%% EDITING
\newcommand{\TR}[1]{\textcolor{red}{TR: #1}}
\newcommand{\TRp}[1]{\textcolor{red}{(TR: #1)}}
% \newcommand{\YG}[1]{\textcolor{orange}{(YG: #1)}}
% \newcommand{\YWT}[1]{\textcolor{green}{(YWT: #1)}}
% \newcommand{\SL}[1]{\textcolor{blue}{SL: #1}}
% \newcommand{\RM}[1]{\textcolor{orange}{RM: #1}}
% \newcommand{\VP}[1]{\textcolor{green}{VP: #1}}
% \newcommand{\TWGR}[1]{\textcolor{orange}{(TWGR: #1)}}
% \newcommand{\OK}[1]{\textcolor{green}{(OK: #1)}}


%%%%%%% TEXT ACRONYMS

\newcommand{\dgps}{\textsc{dgp}s\xspace}
\newcommand{\dgp}{\textsc{dgp}\xspace}
\newcommand{\gps}{\textsc{gp}s\xspace}
\newcommand{\gp}{\textsc{gp}\xspace}
\newcommand{\np}{\textsc{np}\xspace}
\newcommand{\nps}{\textsc{np}s\xspace}
\newcommand{\vae}{\textsc{vae}\xspace}
\newcommand{\vaes}{\textsc{vae}s\xspace}
\newcommand{\iwvae}{\textsc{iwvae}\xspace}
\newcommand{\iwvaes}{\textsc{iwvae}s\xspace}
\newcommand{\svi}{\textsc{svi}\xspace}
\newcommand{\dsvi}{\textsc{dsvi}\xspace}
\newcommand{\iwvi}{\textsc{iwvi}\xspace}
\newcommand{\snr}{\textsc{snr}\xspace}
\newcommand{\snrs}{\textsc{snr}s\xspace}
\newcommand{\dreg}{\textsc{dreg}\xspace}
\newcommand{\clt}{\textsc{clt}\xspace}
\newcommand{\elbo}{\textsc{elbo}\xspace}
\newcommand{\elbos}{\textsc{elbo}s\xspace}
\newcommand{\kld}{KL divergence\xspace}
\newcommand{\jsd}{JS divergence}


%%%%%%% ABBREVIATIONS
\newcommand{\etal}{{et~al.}\ }
\newcommand{\eg}{e.g.\ }
\newcommand{\ie}{i.e.\ }
\newcommand{\nth}{\text{th}}
\newcommand{\pr}{^\prime}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\gauss}{\mathcal{N}}
% \newcommand{\norm}[1]{\left|#1\right|}
% \newcommand{\trace}{\text{tr}}


%%%%%%% REFERENCING
\crefname{appsec}{appendix}{appendices}
\Crefname{appsec}{Appendix}{Appendices}


%%% ICML SETUP

\definecolor{mydarkblue}{rgb}{0,0.08,0.45}
\hypersetup{ %
    pdftitle={},
    pdfauthor={},
    pdfsubject={Proceedings of the International Conference on Machine Learning 2020},
    pdfkeywords={},
    pdfborder=0 0 0,
    pdfpagemode=UseNone,
    colorlinks=true,
    linkcolor=mydarkblue,
    citecolor=mydarkblue,
    filecolor=mydarkblue,
    urlcolor=mydarkblue,
    pdfview=FitH
}

% \hypersetup{
%     colorlinks=true,
%     linktoc=all,     %set to all if you want both sections and subsections linked
%     citecolor=blue,
%     filecolor=blue,
%     linkcolor=blue,
%     anchorcolor = blue,
%     urlcolor=blue  %choose some color if you want links to stand out
% }

% \newcommand\reffig[1]{Figure \ref{fig:#1}}
% \newcommand\refsec[1]{Section \ref{sec:#1}}
% \newcommand\refapp[1]{Appendix \ref{#1}}

% \mathtoolsset{showonlyrefs=true}


%%%%%%% PROOFS

% \newtheorem{definition}{Definition}
% \newtheorem{assumption}{Assumption}
% \newtheorem{remark}{Remark}
% \newtheorem{theorem}{Theorem}
% \newtheorem{proposition}{Proposition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}

\newtheorem{innercustomdefinition}{Definition}
\newenvironment{customdefinition}[1]
  {\renewcommand\theinnercustomdefinition{#1}\innercustomdefinition}
  {\endinnercustomdefinition}

\newtheorem{innercustomtheorem}{Theorem}
\newenvironment{customtheorem}[1]
  {\renewcommand\theinnercustomtheorem{#1}\innercustomtheorem}
  {\endinnercustomtheorem}

\newtheorem{innercustomproposition}{Proposition}
\newenvironment{customproposition}[1]
  {\renewcommand\theinnercustomproposition{#1}\innercustomproposition}
  {\endinnercustomproposition}

\newtheorem{innercustomlemma}{Lemma}
\newenvironment{customlemma}[1]
  {\renewcommand\theinnercustomlemma{#1}\innercustomlemma}
  {\endinnercustomlemma}

\newtheorem{innercustomcorollary}{Corollary}
\newenvironment{customcorollary}[1]
  {\renewcommand\theinnercustomcorollary{#1}\innercustomcorollary}
  {\endinnercustomcorollary}

\newtheorem{innercustomremark}{Remark}
\newenvironment{customremark}[1]
  {\renewcommand\theinnercustomremark{#1}\innercustomremark}
  {\endinnercustomremark}

\newtheorem{innercustomcondition}{Condition}
\newenvironment{customcondition}[1]
  {\renewcommand\theinnercustomcondition{#1}\innercustomcondition}
  {\endinnercustomcondition}


%%%%%%% ALGORITHMS

% \newcommand{\algorithmautorefname}{Algorithm}%
%\newcommand{\theHalgorithm}{\arabic{algorithm}}


%%%%%%% TIKZ

\usetikzlibrary{shapes.geometric, arrows, bayesnet, calc, positioning}


%%%%%%% MATH



%%%%%%% GPs

\DeclareMathOperator{\xbf}{\mathbf{x}}
\DeclareMathOperator{\Xbf}{\mathbf{X}}
\DeclareMathOperator{\ybf}{\mathbf{y}}
\DeclareMathOperator{\Ybf}{\mathbf{Y}}
\DeclareMathOperator{\fbf}{\mathbf{f}}
\DeclareMathOperator{\Fbf}{\mathbf{F}}
\DeclareMathOperator{\hbf}{\mathbf{h}}
\DeclareMathOperator{\Hbf}{\mathbf{H}}
\DeclareMathOperator{\ubf}{\mathbf{u}}
\DeclareMathOperator{\Ubf}{\mathbf{U}}
\DeclareMathOperator{\mbf}{\mathbf{m}}
\DeclareMathOperator{\Sbf}{\mathbf{S}}
\DeclareMathOperator{\zbf}{\mathbf{z}}
\DeclareMathOperator{\Zbf}{\mathbf{Z}}
\DeclareMathOperator{\wbf}{\mathbf{w}}
\DeclareMathOperator{\Wbf}{\mathbf{W}}
\DeclareMathOperator{\bbf}{\mathbf{b}}

\DeclareMathOperator{\kbf}{\mathbf{k}}
\DeclareMathOperator{\Kbf}{\mathbf{K}}
\DeclareMathOperator{\kx}{\mathbf{k_{x}}}
\DeclareMathOperator{\kf}{\mathbf{k_{f}}}
\DeclareMathOperator{\ku}{\mathbf{k_{u}}}
\DeclareMathOperator{\kast}{\mathbf{k_{\ast}}}
\DeclareMathOperator{\Kff}{\mathbf{K_{ff}}}
\DeclareMathOperator{\Kuu}{\mathbf{K_{uu}}}
\DeclareMathOperator{\Kuf}{\mathbf{K_{uf}}}
\DeclareMathOperator{\Kfu}{\mathbf{K_{fu}}}
\DeclareMathOperator{\Kvw}{\mathbf{K_{vw}}}
\DeclareMathOperator{\Kastast}{\mathbf{K_{\ast\ast}}}
\DeclareMathOperator{\Kfast}{\mathbf{K_{f\ast}}}
\DeclareMathOperator{\Kastf}{\mathbf{K_{\ast f}}}
\DeclareMathOperator{\Qff}{\mathbf{Q_{ff}}}
\DeclareMathOperator{\Quu}{\mathbf{Q_{uu}}}
\DeclareMathOperator{\KffT}{\mathbf{K}^\top_{\mathbf{ff}}}
\DeclareMathOperator{\KuuT}{\mathbf{K}^\top_{\mathbf{uu}}}
\DeclareMathOperator{\KufT}{\mathbf{K}^\top_{\mathbf{uf}}}
\DeclareMathOperator{\KfuT}{\mathbf{K}^\top_{\mathbf{fu}}}
\DeclareMathOperator{\KastastT}{\mathbf{K}^\top_{\mathbf{\ast\ast}}}
\DeclareMathOperator{\KfastT}{\mathbf{K}^\top_{\mathbf{f\ast}}}
\DeclareMathOperator{\KastfT}{\mathbf{K}^\top_{\mathbf{\ast f}}}
\DeclareMathOperator{\QffT}{\mathbf{Q}^\top_{\mathbf{ff}}}
\DeclareMathOperator{\QuuT}{\mathbf{Q}^\top_{\mathbf{uu}}}
\DeclareMathOperator{\Kffinv}{\mathbf{K}^{-1}_{\mathbf{ff}}}
\DeclareMathOperator{\Kuuinv}{\mathbf{K}^{-1}_{\mathbf{uu}}}
\DeclareMathOperator{\Kufinv}{\mathbf{K}^{-1}_{\mathbf{uf}}}
\DeclareMathOperator{\Kfuinv}{\mathbf{K}^{-1}_{\mathbf{fu}}}
\DeclareMathOperator{\Kastastinv}{\mathbf{K}^{-1}_{\mathbf{\ast\ast}}}
\DeclareMathOperator{\Kfastinv}{\mathbf{K}^{-1}_{\mathbf{f\ast}}}
\DeclareMathOperator{\Kastfinv}{\mathbf{K}^{-1}_{\mathbf{\ast f}}}
\DeclareMathOperator{\Qffinv}{\mathbf{Q}^{-1}_{\mathbf{ff}}}
\DeclareMathOperator{\Quuinv}{\mathbf{Q}^{-1}_{\mathbf{uu}}}
\DeclareMathOperator{\thetabf}{\bm{\theta}}
\DeclareMathOperator{\omegabf}{\bm{\omega}}
\DeclareMathOperator{\dxbf}{\text{d}\mathbf{x}}
\DeclareMathOperator{\dfbf}{\text{d}\mathbf{f}}
\DeclareMathOperator{\dFbf}{\text{d}\mathbf{F}}
\DeclareMathOperator{\dubf}{\text{d}\mathbf{u}}
\DeclareMathOperator{\dzbf}{\text{d}\mathbf{z}}
\DeclareMathOperator{\dZbf}{\text{d}\mathbf{Z}}
\DeclareMathOperator{\dwbf}{\text{d}\mathbf{w}}
\DeclareMathOperator{\dWbf}{\text{d}\mathbf{W}}
\DeclareMathOperator{\db}{\text{d}b}
\DeclareMathOperator{\dbbf}{\text{d}\mathbf{b}}

\newcommand{\bJ}{\mathbf{J}}
\newcommand{\Kpp}{\mathbf{K}_{\mathbf {\phi \phi}}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bff}{\mathbf f}
\newcommand{\bk}{\mathbf k}
\newcommand{\bfm}{\mathbf m}
\newcommand{\bX}{\mathbf X}
\newcommand{\by}{\mathbf y}
\newcommand{\bx}{\mathbf x}
\newcommand{\bu}{\mathbf u}
\newcommand{\bv}{\mathbf v}
\newcommand{\bR}{\mathbf R}
\newcommand{\bs}{\mathbf s}
\newcommand{\bS}{\mathbf S}
\newcommand{\bZ}{\mathbf Z}
\newcommand{\bzero}{\mathbf 0}
\newcommand{\dee}{\,\textrm{d}}
\newcommand{\given}{\,|\,}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calGP}{\mathcal{GP}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calI}{\mathcal{I}}

\newcommand{\Zhat}{\hat{Z}}
\newcommand{\ztilde}{\tilde{z}}
\newcommand{\ftilde}{\tilde{f}}

\newcommand{\x}{\mathbf{x}}
\newcommand{\z}{\mathbf{z}}
\renewcommand{\L}{\mathbf{L}}
\renewcommand{\l}{{\ell}}
\newcommand{\bl}{{\boldsymbol\ell}}
\renewcommand{\u}{\mathbf{u}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\h}{\mathbf{h}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\e}{\mathbf{e}}
\renewcommand{\a}{\mathbf{a}}
\renewcommand{\t}{\mathbf{t}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\g}{ {\mathbf{g} }}
\newcommand{\m}{{\mathbf{m}}}
\newcommand{\mw}{{\mathbf{m}_w}}
\newcommand{\bg}{ {\boldsymbol\gamma}  }
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\K}{\mathbf{K}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\Qf}{\mathbf{Q}_{\mathbf{f}}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\Mf}{\mathbf{M}_{\mathbf{f}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\tL}{{\tilde{\mathcal{L}}}}
\newcommand{\0}{\mathbf{0}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\dX}{\dot{\mathcal{X}}}
\newcommand{\w}{{\boldsymbol{\sigma}}}
\newcommand{\s}{{\sigma}}
\renewcommand{\S}{{\mathbf{S}}}
\newcommand{\bo}{\boldsymbol{\omega}}
\newcommand{\bO}{\boldsymbol{\Omega}}
\renewcommand{\o}{{\omega}}
\renewcommand{\O}{{\Omega}}
\newcommand{\bmu}{{\boldsymbol{\mu}}}
\newcommand{\btheta}{{\boldsymbol{\theta}}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\tV}{\widetilde{V}}
\newcommand{\tU}{\widetilde{U}}
\newcommand{\tu}{\widetilde{\mathbf{u}}}
\newcommand{\tv}{\widetilde{\mathbf{v}}}
\newcommand{\tS}{\tilde{\Sigma}}
\newcommand{\tm}{\tilde{\mathbf{m}}}
\newcommand{\tmu}{\tilde{\boldsymbol{\mu}}}
\newcommand{\tg}{\tilde{\bg}}
\newcommand{\tf}{\tilde{f}}
\def\w{\mathbf{w}}

\newcommand{\Lb}{\mathcal{L}}
% \newcommand{\Z}{\mathbf{Z}}
% \newcommand{\W}{\mathbf{W}}

\newcommand{\tKf}{\tilde{K}_{f mm}}
\newcommand{\tKw}{\tilde{K}_{w mm}}
\newcommand{\tKg}{\tilde{K}_{\gamma mm}}
\newcommand{\tKo}{\tilde{K}_{\omega mm}}
\newcommand{\tKb}{\tilde{K}_{\beta mm}}

\newcommand{\Xt}{{\mathbf{X}_t}}
\newcommand{\XT}{{\mathbf{X}_T}}
\newcommand{\XTs}{{\mathbf{X}_T^{(s)}}}

\newcommand{\Zg}{{\mathbf{Z}_g}}
\newcommand{\Zf}{{\mathbf{Z}_\mathbf{f}}}
\newcommand{\Zft}{{\mathbf{Z}_\mathbf{f}^t}}
\newcommand{\Zfs}{{\mathbf{Z}_\mathbf{f}^s}}
\newcommand{\Ug}{{\mathbf{U}_g}}
\newcommand{\Uf}{{\mathbf{U}_\mathbf{f}}}

\newcommand{\ufj}{{\mathbf{u}_{\mathbf{f}j}}}

\newcommand{\ug}{{\mathbf{u}_g}}
\newcommand{\uw}{{\mathbf{u}_w}}
\newcommand{\us}{{\mathbf{u}_\sigma}}
\newcommand{\uo}{{\mathbf{u}_\omega}}
\newcommand{\ub}{{\mathbf{u}_\beta}}
\newcommand{\uf}{{\mathbf{u}_\mathbf{f}}}
\newcommand{\mf}{{\mathbf{m}_\mathbf{f}}}
\newcommand{\Sf}{{\mathbf{S}_\mathbf{f}}}
\newcommand{\mo}{{\mathbf{m}_\omega}}
\newcommand{\So}{{\mathbf{S}_\omega}}
\newcommand{\mb}{{\mathbf{m}_\beta}}
\newcommand{\Sb}{{\mathbf{S}_\beta}}
\newcommand{\mg}{{\mathbf{m}_g}}
\newcommand{\Sg}{{\mathbf{S}_g}}
\newcommand{\Sw}{{\mathbf{S}_w}}
\newcommand{\pbg}{\Phi(\bg)}
\newcommand{\pg}{\phi(\g)}
\newcommand{\Sn}{\sigma_n^2}
\newcommand{\fl}{\mathcal{L}_1}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\newcommand{\Qp}{ Q^{p_\omega}}
\newcommand{\piq}{\pi^q}

\newcommand{\bphi}{\boldsymbol\phi}
\newcommand{\balpha}{\boldsymbol\alpha}
\newcommand{\bbeta}{\boldsymbol\beta}
\newcommand{\bSigma}{\boldsymbol\Sigma}
\newcommand{\infint}{\int_{-\infty}^\infty}
\newcommand{\kron}{\raisebox{1pt}{\ensuremath{\:\otimes\:}}}

\newcommand{\matern}{{Mat\'ern}\xspace}
\newcommand{\maternonetwo}{{Mat\'ern-\ensuremath{\tfrac{1}{2}}}\xspace}
\newcommand{\maternthreetwo}{{Mat\'ern-\ensuremath{\tfrac{3}{2}}}\xspace}
\newcommand{\maternfivetwo}{{Mat\'ern-\ensuremath{\tfrac{5}{2}}}\xspace}

\newcommand{\closer}[3]{{\kern-#1ex{#2}\kern-#3ex}}

\newcommand\PS[1]{{\left \langle #1 \right \rangle}_{\! \cH}}
\newcommand\PSi[2]{{ \left \langle #1 \right \rangle}_{\! #2}}


\def\changemargin#1#2{\list{}{\rightmargin#2\leftmargin#1}\item[]}
\let\endchangemargin=\endlist 


%%%%%%% MATH OPERATORS & SYMBOLS

\newcommand{\DKL}{D_{\text{KL}}\infdivx}
\newcommand{\DJS}{D_{\text{JS}}\infdivx}

\newcommand{\ELBO}[1]{\text{ELBO}(#1)}

\DeclareMathOperator{\gradphi}{\nabla_{\phi}}
\DeclareMathOperator{\gradtheta}{\nabla_{\theta}}
\DeclareMathOperator{\gradpsi}{\nabla_{\psi}}

\newcommand{\xbest}{\mathbf{\vx}^{+}}
\newcommand{\xstar}{\mathbf{\vx}^{*}}
\newcommand{\ystar}{\mathbf{\vy}^{*}}
\DeclareMathOperator*{\T}{^\intercal}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\pluseq}{\mathrel{+}=}

\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\mean}{mean}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\vect}{vec}


%%%%%%% SETS
\DeclareMathOperator*{\setunion}{ \cup }
\DeclareMathOperator*{\Setunion}{ \bigcup }
\DeclareMathOperator*{\setintersect}{ \cap }
\DeclareMathOperator*{\Setintersect}{ \bigcap }
\DeclareMathOperator*{\setand}{ \wedge }
\DeclareMathOperator*{\Setand}{ \bigwedge }
\mathchardef\mhyphen="2D


%%%%%%% EXPECTATIONS & VARIANCES
\DeclareMathOperator{\E}{\mathbb{E}}
\newcommand{\ex}[1]{{\mathbb E}\left[ #1 \right]}
\newcommand{\exc}[2]{{\mathbb E}\left[ #1 \,\middle \vert\, #2 \right]}
\newcommand{\exs}[2]{{\mathbb E_{#1}}\left[ #2 \right]}
\newcommand{\vars}[2]{{\mathbb V_{#1}}\left[ #2 \right]}
\newcommand{\excs}[3]{{\mathbb E_{#1}}\left[ #2 \,\middle \vert\, #3 \right]}

\newcommand{\xxcomment}[4]{\textcolor{#1}{[$^{\textsc{#2}}_{\textsc{#3}}$ #4]}}
\newcommand{\sanyam}[1]{\xxcomment{blue}{S}{K}{#1}}

==> include/custom_aabi2023.tex <==
%%%%%%% LAYOUT

% \usepackage[
%   paper  = letterpaper,
%   left   = 1.65in,
%   right  = 1.65in,
%   top    = 1.0in,
%   bottom = 1.0in,
%   ]{geometry}
% Set the typeface to Times Roman
% \usepackage{times}
% Changes typeface to Bitstream Charter
% \usepackage[bitstream-charter]{mathdesign}
% \usepackage{include/jmlr2e}


% \usepackage{titletoc}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{colortbl}

% \newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
% \newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut


% \definecolor{azure}{rgb}{0.0, 0.5, 1.0}
% \definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
% \definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}

% \newtheorem{innercustomassumption}{Assumption}
% \newenvironment{customassumption}[1]
%   {\renewcommand\theinnercustomassumption{#1}\innercustomassumption}
%   {\endinnercustomassumption}
  
% % \newcommand\defines{\stackrel{\mathclap{\normalfont\mbox{\tiny def}}}{=}}
% \newcommand\defines{\,\dot{=}\,}





\usepackage{microtype}
\usepackage{graphicx}
% \usepackage{subfigure}
\usepackage{booktabs} % for professional tables

\usepackage{hyperref}
%\hypersetup{colorlinks=True,urlcolor=magenta}
\usepackage{url}
\usepackage{wrapfig}


% {\arabic{algorithm}}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}

\usepackage[title]{appendix}
% \usepackage{natbib}
\usepackage[nameinlink]{cleveref} % 

\newtheorem{hyp}{Hypothesis} 
% \newtheorem{thm}{Theorem}
% \newtheorem{lemma}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{defn}{Definition}
\newtheorem{mydef}{Definition}
\newtheorem{conj}{Conjecture}
%\newtheorem{remark}{Remark}
% \newtheorem{ex}{Example}
\newtheorem{exercise}{Exercise}




\def \C{\mathcal{C}}
\def \P{\mathbf{P}}
\def \So{\mathcal{S}}
\def \cZ{\boldsymbol{Z}}
\def \cS{\boldsymbol{S}}
\def \cM{\boldsymbol{M}}
\def \PD{\text{PD}}
\newcommand{\bigcdot}{\boldsymbol{\cdot}}
\def \bx{\boldsymbol{x}}
\def \bnu{\boldsymbol{\nu}}
\def \by{\boldsymbol{y}}
\def \bz{\boldsymbol{z}}
\def \bm{\boldsymbol{m}}
\def \bv{\boldsymbol{v}}
\def \bp{\boldsymbol{p}}
\def \bh{\boldsymbol{h}}
\def \bs{\boldsymbol{s}}
%\def \bS{\boldsymbol{S}}
\def \bu{\boldsymbol{u}}
\def \bG{\boldsymbol{G}}
\def \bk{\boldsymbol{k}}
\def \bv{\boldsymbol{v}}
\def \bb{\boldsymbol{b}}
\def \bd{\boldsymbol{d}}
\def \bg{\boldsymbol{g}}
\def \bq{\boldsymbol{q}}
\def \bm{\boldsymbol{m}}
\def \bw{\boldsymbol{w}}
\def \be{\boldsymbol{e}}
\def \br{\boldsymbol{r}}
\def \bR{\boldsymbol{R}}
\def \ba{\boldsymbol{a}}
\def \bA{\boldsymbol{A}}
\def \bAA{\mathbf{\mathbb{A}}}
\def \bK{\boldsymbol{K}}
\def \bB{\boldsymbol{B}}
\def \bV{\boldsymbol{V}}
\def \bJ{\boldsymbol{J}}
\def \bU{\boldsymbol{U}}
\def \bC{\boldsymbol{C}}
\def \bZ{\boldsymbol{Z}}
\def \bD{\boldsymbol{D}}
\def \bW{\boldsymbol{W}}
\def \bt{\boldsymbol{t}}
\def \bH{\boldsymbol{H}}
\def \bX{\boldsymbol{X}}
\def \bQ{\boldsymbol{Q}}
\def \bI{\boldsymbol{I}}
\def \bPhi{\boldsymbol{\Phi}}
\def \bphi{\boldsymbol{\phi}}
\def \bSigma{\boldsymbol{\Sigma}}
\def \balpha{\boldsymbol{\alpha}}
\def \bbeta{\boldsymbol{\beta}}


\def \s{\textbf{s}}
\def \t{\textbf{t}}
\def \z{\textbf{z}}
\def \x{\textbf{x}}
\def \BP{\boldsymbol{P}}
\def \BE{\boldsymbol{E}}
\def \gepsilon{\boldsymbol{\epsilon}}





% \def\R{{\mathbb R}}
% \def\E{{\mathbb E}}
\def\Pr{{\mathbb P}}
\def\Indic{\mathbbm{1}} 
\def \pa{{\mathrm{pa}}}
\def \Epsilon{\mathcal{E}}
\def \EPSILON{E}


\newcommand{\Z}[0] {{ \mathbb{Z} }}
\newcommand{\N}[0] {{ \mathbb{N} }}
\newcommand{\Expect}[0] {{ \mathbb{E} }}
\newcommand{\MaxExp}[0] {{ \mathbb{M} }}
\newcommand{\D}[0] {{ \mathcal{D} }}
\newcommand{\dg}[0] {{ \dagger }}
\newcommand{\Cl}[0] {{ \mathcal{C} }}
\newcommand{\G}[0] {{ \mathcal{G} }}
\newcommand{\HH}[0] {{ \mathcal{H} }}
\newcommand{\Pa}[0] {{ \mathcal{P} }}
\newcommand{\W}[0] {{ \mathcal{W} }}
\newcommand{\M}[0] {{ \mathcal{M} }}
\newcommand{\richb}[1]{\textcolor{red}{#1}}
\newcommand{\imtiaz}[1]{\textcolor{magenta}{#1}}
\newcommand{\rbal}[1]{\textcolor{blue}{#1}}


\newcommand{\out}{z}
\newcommand{\im}{\text{Im}}
\newcommand{\Aff}{\text{Aff}}
\newcommand{\adj}{\text{adj}}
\newcommand{\spann}{\text{span}}

%KK
\usepackage{include/DefinitionsO}
% \newcommand{\T}{^\top}
\newcommand{\hx}{{\hat x}}
\newcommand{\hy}{{\hat y}}
\newcommand{\hdelta}{{\hat \delta}}
\newcommand{\cx}{{\check x}}
\newcommand{\hLcal}{{\hat \Lcal}}
% \newcommand{\tf}{{\tilde f}}
\newcommand{\tphi}{{\tilde \phi}}
\newcommand{\bCcal}{{\bar \Ccal}}
\newcommand{\tCcal}{{\tilde \Ccal}}
\newcommand{\tpsi}{{\tilde \psi}}
\newcommand{\td}{{\tilde d}}
\newcommand{\tLcal}{{\tilde \Lcal}}
\newcommand{\amax}{a_{\text{max}}}
\newcommand{\tIcal}{{\tilde \Ical}}
\newcommand{\bdelta}{{\bar \delta}}
\newcommand{\hA}{{\hat A}}
\newcommand{\hXcal}{{\hat \Xcal}}
\newcommand{\ha}{{\hat a}}
\newcommand{\hT}{{\hat T}}
\newcommand{\hIcal}{{\hat \Ical}}
\newcommand{\bxi}{{\bar \xi}}
\newcommand{\hXi}{{\hat \Xi}}
\newcommand{\hZcal}{{\hat \Zcal}}
\newcommand{\tbeta}{{\tilde \beta}}
\newcommand{\Lc}{L_{\text{cont}}}
\newcommand{\xp}{x^{+}}
\newcommand{\xpp}{x^{++}}
\newcommand{\xn}{x^{-}}
\newcommand{\hw}{{\hat w}}
\newcommand{\ty}{{\tilde y}}
\newcommand{\tYcal}{{\tilde \Ycal}}
\newcommand{\hp}{{\hat p}}
\newcommand{\bYcal}{{\bar \Ycal}}
\newcommand{\tx}{{\tilde x}}
\newcommand{\hZ}{{Z_\bS}}
\newcommand{\yp}{y^{+}}
\newcommand{\tW}{{\tilde W}}
\newcommand{\bbx}{{\bar x}}
% \newcommand{\bS}{{\bar S}}
\newcommand{\tZ}{{Z_S}}
\newcommand{\bby}{{\bar y}}
